When is a Convolutional Filter Easy To Learn?

We analyze the convergence of (stochastic) gradient descent algorithm for learning a convolutional filter with Rectified Linear Unit (ReLU) activation function. Our analysis does not rely on any specific form of the input distribution and our proofs only use the definition of ReLU, in contrast with previous works that are restricted to standard Gaussian input. We show that (stochastic) gradient descent with random initialization can learn the convolutional filter in polynomial time and the convergence rate depends on the smoothness of the input distribution and the closeness of patches. To the best of our knowledge, this is the first recovery guarantee of gradient-based algorithms for convolutional filter on non-Gaussian input distributions. Our theory also justifies the two-stage learning rate strategy in deep neural networks. While our focus is theoretical, we also present experiments that illustrate our theoretical findings.

==> one_patch_rate.tex <==
%\simon{We may need to rewrite this paragraph to emphasize on the smoothness of the distribution.}
In the previous section we showed if the distribution is regular and the weights are initialized appropriately, gradient descent recovers the true weights when it converges.
In practice we also want to know how many iterations are needed.
%In this section, we consider the convergence rate of gradient descent. 
To characterize the convergence rate, we need some quantitative assumptions.
We note that  different set of assumptions will lead to different rates and ours is only one possible choice.  
In this paper we use the following quantities.
\begin{defn}[The Largest and the Least Eigenvalue Values of the Second Moment on Intersection of two Half Spaces]\label{def:eigens_and_angle}
	For $\phi \in \left[0,\pi \right]$,
	 define\begin{align*} 
		\gamma(\phi)  = \min_{\vect{w}: \angle \vect{w},\vect{w}_*\le \phi}
		\lambda_{\min}\left(\mat{A}_{\vect{w},\vect{w}_*}\right), \quad 
	L(\phi)  = \max_{\vect{w}: \angle \vect{w},\vect{w}_*\le \phi}
	\lambda_{\max}\left(\mat{A}_{\vect{w},\vect{w}_*}\right),
	\end{align*}
\end{defn}
These two conditions quantitatively characterize the smoothness of the input distribution.
For a given angle $\phi$, if the difference between $\gamma(\phi)$ and $L(\phi)$ is large then there is one direction has large probability mass and one direction has small probability mass, meaning the input distribution is not smooth.
On the other hand, if $\gamma(\phi)$ and $L(\phi)$ are close, then all directions have similar probability mass, which means the input distribution is smooth.
The smoothest input distributions are rotationally invariant distributions (e.g.  standard Gaussian) which have $\gamma(\phi) = L(\phi)$.
For analogy, we can think of $L(\phi)$ Lipschitz constant of the gradient and $\gamma(\phi)$ as the strong convexity parameter in the optimization literature but here we also allow they change with the angle.
Also observe that when $\phi = \pi$, $\gamma(\phi) = L(\phi) = 0$ because the intersection has measure $0$ and both $\gamma(\phi)$ and $L(\phi)$ are monotonically decreasing.

Our next assumption is on the growth of $\mat{A}_{\vect{w},-\vect{w}_*}$.
Note that when $\theta\left(\vect{w},\vect{w}_*\right) = 0$, then $\mat{A}_{\vect{w},-\vect{w}_*} = \mat{0}$ because the intersection between $\vect{w}$ and $-\vect{w}_*$ has $0$ measure.  Also, $\mat{A}_{\vect{w},-\vect{w}_*}$ grows as the angle between $\vect{w}$ and $\vect{w}_*$ becomes larger.
We assume the operator norm of $\mat{A}_{\vect{w},-\vect{w}_*}$ increases smoothly with respect to the angle.
\begin{asmp}\label{asmp:lispchitz_growth}
Let $L_{\gele}\left(\phi\right) = \max_{\vect{w},\theta\left(\vect{w},\vect{w}_*\right) \le \phi} \lambda_{\max}\left(\mat{A}_{\vect{w},-\vect{w}_*}\right)$.
We assume there exists $\beta > 0$ that for $0\le \phi \le \pi /2$, $L_{\gele}\le \beta\phi$.
\end{asmp} 
Theorem~\ref{thm:rot_invar_beta} shows this condition is true for rotational invariant distributions, e.g., Gaussian.
It still holds for a large class of input distribution which has compact support and bounded probability density.
Now we are ready to state the convergence rate.
\begin{thm}\label{thm:one_patch_convergence_rate}
Suppose the initialization $\vect{w}_0$ satisfies $\norm{\vect{w}_0-\vect{w}_*}_2 < \norm{\vect{w}_*}_2$.
Denote $\phi_t = \arcsin\left(\frac{\norm{\vect{w_t}-\vect{w}_*}_2}{\norm{\vect{w}_*}_2}\right)$
then if step size is set as $0 \le \eta_t \le \min_{0 \le \phi_t \le \frac{\pi}{2}} \frac{\gamma(\phi_t)}{2\left(L(\phi_t)+2\beta\right)^2}$, we have for $t=1,2,\ldots$\begin{align*}
	\norm{\vect{w}_{t+1}-\vect{w}_*}_2^2 \le \left(1-\frac{\eta_t\gamma\left(\phi_t\right)}{2}\right)\norm{\vect{w}_t - \vect{w}_*}_2^2.
\end{align*}
\end{thm}
Note both $\gamma(\phi)$ and $L(\phi)$ increases as $\phi$ decreases so we can choose a constant step size $\eta_t = \Theta\left(\frac{\gamma(\phi_0)}{\left(L(0)+\beta\right)^2}\right)$.
This theorem implies that we can find the $\epsilon$-close solution of $\vect{w}_*$ in $O\left(\frac{\left(L(0)+\beta\right)^2}{\gamma^2(\phi_0)}\log\left(\frac{1}{\epsilon}\right)\right)$ iterations.
It also suggests a direct relation between the smoothness of the distribution and the convergence rate.
For smooth distribution where $\gamma(\phi)$ and $L(\phi)$ are close and $\beta$ is small then $\frac{\left(L(0)+\beta\right)^2}{\gamma^2(\phi_0)}$ is relatively small and we need fewer iterations.
On the other hand, if $L(\phi)$ or $\beta$ is much larger than $\gamma(\phi)$, we will need more iterations.
We verify this intuition in Section~\ref{sec:exp}.
%Now with these insights at hand, we can proceed to analyze the convolution filter.

If we are able to choose the step sizes adaptively $\eta_t = \Theta\left(\frac{\gamma(\phi_t)}{\left(L(\phi_t)+\beta\right)^2}\right)$, like using methods proposed by~\citet{lin2014adaptive}, we may improve the computational complexity to $O\left(\max_{\phi \le \phi_0}\frac{\left(L(\phi)+\beta\right)^2}{\gamma^2\left(\phi\right)}\log\left(\frac{1}{\epsilon}\right)\right)$.
This justifies the use of two-stage learning rate strategy proposed by~\citet{he2016deep,szegedy2017inception} where at the begging we need to choose learning to be small because $\frac{\gamma(\phi_0)}{2\left(L(\phi_0)+2\beta\right)^2}$ is small and later we can choose a large learning rate because as the angle between $\vect{w}_t$ and $\vect{w}_*$ becomes smaller, $\frac{\gamma(\phi_t)}{2\left(L(\phi_t)+2\beta\right)^2}$ becomes bigger.


The proof of this theorem relies our observation from Section~\ref{sec:one_patch} and the quantitative assumptions.
The theorem requires the initialization satisfying $\norm{\vect{w}_0-\vect{w}_*}_2 < \norm{\vect{w}_*}_2$, which can be achieved by random initialization with constant success probability.
See Section~\ref{sec:init} for a detailed discussion.
%\simon{This may be very important implication, do we need to expand it?}\yuandong{Yes. Go ahead. This might explain different choice of learning rate depends on data distribution. The ratio $\gamma(\phi_t) / L(\phi_t)$ is dataset-dependent and important.}


%\begin{figure}
%	\centering
%	\includegraphics[width=0.7\linewidth, angle = 270]{figs/rot_invar}
%	\caption{}
%	\label{fig:rot_invar}
%\end{figure}



%\noindent Now we consider the convergence rate of stochastic gradient descent.
%\begin{thm}\label{thm:one_patch_rate_sgd}
%Denote $r_0 = \norm{\vect{w}_0-\vect{w}_*}_2$, $\phi_0 = \arcsin\left(\frac{r_0}{\norm{\vect{w}_*}_2}\right)$	and $\phi_1 = \frac{\phi_0 + \pi/2}{2}$.
%For $\epsilon$ sufficiently small \footnote{We only need it to be smaller than some rational function of problem depend parameter and $\log(1/\delta)$.}, if $\eta = \Theta \left(\frac{\epsilon^2\gamma(\phi_1)\norm{\vect{w}_*}_2^2}{B^2}\right)$, then we have in $T = O\left(\frac{B^2}{\epsilon^2\gamma(\phi_1)^2\norm{\vect{w}_*}_2^2} \log\left(\frac{\norm{\vect{w}_0-\vect{w}_*}}{\epsilon\delta \norm{\vect{w}_*}_2
%	}\right)\right)$ iterations, with probability at least $1-\delta$ we have $
%	\norm{\vect{w}_T - \vect{w}_*}_2 \le \epsilon\norm{\vect{w}_*}_2.$
%\end{thm}

